Align-gram : Rethinking the Skip-gram Model for Protein Sequence Analysis

Background: The inception of next generations sequencing technologies have exponentially increased the volume of biological sequence data. Protein sequences, being quoted as the `language of life', has been analyzed for a multitude of applications and inferences. Motivation: Owing to the rapid development of deep learning, in recent years there have been a number of breakthroughs in the domain of Natural Language Processing. Since these methods are capable of performing different tasks when trained with a sufficient amount of data, off-the-shelf models are used to perform various biological applications. In this study, we investigated the applicability of the popular Skip-gram model for protein sequence analysis and made an attempt to incorporate some biological insights into it. Results: We propose a novel $k$-mer embedding scheme, Align-gram, which is capable of mapping the similar $k$-mers close to each other in a vector space. Furthermore, we experiment with other sequence-based protein representations and observe that the embeddings derived from Align-gram aids modeling and training deep learning models better. Our experiments with a simple baseline LSTM model and a much complex CNN model of DeepGoPlus shows the potential of Align-gram in performing different types of deep learning applications for protein sequence analysis.

==> old_tables.tex <==

\begin{table}[h]
\caption{Task Results : DNA-Binding-Protein Prediction (Binary Classification)}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
Embedding & Precision & Recall & F1 & Accuracy \\ \hline
One Hot Encodding & 48.105 $\pm$ 24.33 & 60.43 $\pm$ 31.521 & 53.241 $\pm$26.931 & 59.892 $\pm$ 6.303 \\ \hline
Blosum62 & 55.606 $\pm$ 1.911 & 82.151 $\pm$ 3.942 & 66.301 $\pm$ 2.429 & 58.28 $\pm$ 2.775 \\ \hline
Skip-gram & 57.83 $\pm$ 2.569 & 55.914 $\pm$ 7.843 & 56.647 $\pm$ 4.713 & 57.634 $\pm$ 2.75 \\ \hline
Align-gram & \textbf{61.66 $\pm$ 4.166} & \textbf{85.591 $\pm$ 3.233} & \textbf{71.603 $\pm$ 3.365} & \textbf{65.914 $\pm$ 5.085} \\ \hline
\end{tabular}
\end{table}


\begin{table}[h]
\caption{Task Results : Remote Homology Detection (Multiclass Classification)}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Embedding & Top-1 Acc. & Top-5 Acc. & Top-10 Acc. \\ \hline
One Hot Encodding & 17.57 $\pm$ 3.861 & 40.641 $\pm$ 8.546 & 59.183 $\pm$ 6.81 \\ \hline
Blosum62 & 18.04 $\pm$ 2.619 & 41.335 $\pm$ 6.968 & 56.706 $\pm$ 4.303 \\ \hline
Skip-gram & 19.847 $\pm$ 3.033 & 52.456 $\pm$ 3.373 & 70.032 $\pm$ 2.245 \\ \hline
Align-gram & \textbf{24.308 $\pm$ 2.055} & \textbf{55.332 $\pm$ 2.056} & \textbf{71.702 $\pm$ 3.774} \\ \hline
\end{tabular}
\end{table}


\begin{table}[h]
\caption{Task Results : Protein Stability Prediction (Regression)}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Embedding & MSE & MAE & $\rho$ \\ \hline
One Hot Encodding & 0.17 $\pm$ 0.003 & 0.309 $\pm$ 0.003 & 0.781 $\pm$ 0.005 \\ \hline
Blosum62 & 0.195 $\pm$ 0.004 & 0.345 $\pm$ 0.005 & 0.743 $\pm$ 0.007 \\ \hline
Skip-gram & 0.202 $\pm$ 0.009 & 0.347 $\pm$ 0.007 & 0.73 $\pm$ 0.012 \\ \hline
Align-gram & \textbf{0.145 $\pm$ 0.003} & \textbf{0.285 $\pm$ 0.004} & \textbf{0.815 $\pm$ 0.005} \\ \hline
\end{tabular}
\end{table}

\begin{table}[h]
\caption{Task Results : Protein Secondary Structure Prediction (seq2seq)}
\centering
\begin{tabular}{|c|c|c|}
\hline
Embedding & 3 Class Accuracy & 8 Class Accuracy \\ \hline
One Hot Encodding & 50.156 $\pm$ 1.683 & 26.801 $\pm$ 1.725 \\ \hline
Blosum62 & 47.372 $\pm$ 1.144 & 25.062 $\pm$ 1.103 \\ \hline
Skip-gram & 46.923 $\pm$ 3.41 & 27.579 $\pm$ 1.569 \\ \hline
Align-gram & \textbf{54.884 $\pm$ 0.721} & \textbf{32.66 $\pm$ 1.643} \\ \hline
\end{tabular}
\end{table}

best paper ever :  https://sci-hub.st/https://onlinelibrary.wiley.com/doi/abs/10.1002/pmic.201900335

